Dissecting Multimodality in VideoQA Transformer Models by Impairing Modality Fusion

While VideoQA Transformer models demonstrate competitive performance on standard benchmarks, the reasons behind their success are not fully understood. Do these models capture the rich multimodal structures and dynamics from video and text jointly? Or are they achieving high scores by exploiting biases and spurious features? Hence, to provide insights, we design $\textit{QUAG}$ (QUadrant AveraGe), a lightweight and non-parametric probe, to conduct dataset-model combined representation analysis by impairing modality fusion. We find that the models achieve high performance on many datasets without leveraging multimodal representations. To validate QUAG further, we design $\textit{QUAG-attention}$, a less-expressive replacement of self-attention with restricted token interactions. Models with QUAG-attention achieve similar performance with significantly fewer multiplication operations without any finetuning. Our findings raise doubts about the current models' abilities to learn highly-coupled multimodal representations. Hence, we design the $\textit{CLAVI}$ (Complements in LAnguage and VIdeo) dataset, a stress-test dataset curated by augmenting real-world videos to have high modality coupling. Consistent with the findings of QUAG, we find that most of the models achieve near-trivial performance on CLAVI. This reasserts the limitations of current models for learning highly-coupled multimodal representations, that is not evaluated by the current datasets (project page: https://dissect-videoqa.github.io ).

==> main_content/dataset_analysis.tex <==
Shortcuts are spurious features in the data that are easier to learn than the \emph{core}-features necessary for generalization \citep{geirhos2020shortcut, murali2023shortcut}. We posit that consistent shortcuts in the dataset enable the models to achieve high accuracy without even learning from the temporal video sequence. 

 % We take an example from NExT-QA (\citet{xiao2021next}) that contains 47,692 5-way multiple choice questions divided into temporal, causal and descriptive categories to motivate that performance on temporal questions might not be representative of temporal understanding. 

% For an 5-way multiple-choice question, the chance accuracy is ideally $ 20\% $. However, in reality, the likeliness of all the options is not the same. Since the the incorrect options are (semi-)automatically curated, inadvertent shortcuts are created that discount temporal understanding, allowing the models to operate in eliminative strategy to achieve high accuracy. For example, consider the following temporal question from NExT-QA (\citet{xiao2021next}), \emph{"What did the person do after the animal started sniffing the black item on the bed?"} with answer-options as (a) jump on it, (b) changing the diaper, (c) remove black item (d) playing with toy (e) move away. Since diaper and toy do not exist in the video, (b) and (d) can be eliminated based on the static visual information. Also, both (b) and (d) are syntactically incorrect answers and can be also eliminated by language understanding alone. Further, many action categories, including jump, can be inferred without temporal understanding (\citet{sevilla2021only}). Hence, based on only static and linguistic shortcuts, the probable answer pool is reduced to (c) and (e). Note that in evaluating these shortcuts, we did not gather any information from the word \textit{after} in the question or from the temporal sequence of the frames. Hence, performance on temporal questions might not be indicative of temporal understanding. 

Ideally, for an 5-way multiple-choice question, the chance accuracy is $ 20\% $. However, in reality, the likeliness of all the options is not the same. Since in VideoQA datasets the incorrect options are (semi-)automatically curated, inadvertent shortcuts are created that discount temporal understanding, allowing the models to operate in option elimination strategy to achieve high accuracy \citep{chao2018being}. For example, consider the following temporal question from NExT-QA \citep{xiao2021next}, \emph{"What did the person do after the animal started sniffing the black item on the bed?"} with answer-options as (a) jump on it, (b) changing the diaper, (c) remove black item (d) playing with toy (e) move away. Since diaper and toy do not exist in the video, (b) and (d) can be eliminated based on the static visual information. Also, both (b) and (d) are syntactically incorrect answers and can be also eliminated by language understanding alone. Further, many action categories, including jump, can be inferred without temporal understanding \citep{sevilla2021only}. Hence, based on only static and linguistic shortcuts, the probable answer pool is reduced to (c) and (e). Note that in evaluating these shortcuts, we did not gather any information from the word \textit{after} in the question or from the temporal sequence of the frames. Hence, performance on temporal questions might not be indicative of temporal understanding. 

Likewise, eliminative strategy in the entire vocabulary set exists in open-ended VideoQA datasets. In addition, in open-ended datsets, ambiguities can exist in either the question, answer or both. 
For example, in ActivityNet-QA \citep{yu2019activityqa}, \emph{cook food} and \emph{make spaghetti} are treated distinct answers, which is an example of ambiguity in answer since both the answers might be correct at different levels of abstraction. Similarly, ambiguity in question can arise in, for example, in temporal questions like \emph{"What did the person do after <EVENT>?"}. This is because temporal prepositions only encode chronology. Hence, multiple correct answers can exist but only one of them is annotated with a single ground-truth answer. 
Therefore, ambiguities makes learning from core-features more noisy; inadvertently increases the reliance on learning from the spurious features.


% Assessing shortcuts can be challenging due to misleading features within and between modalities. To address this, we use treatment of shortcuts by \citet{murali2023shortcut}. They present a combined model and dataset dependent treatment of shortcuts that not all spurious correlations, but only the ones in the dataset that, for a given model, are easier to learn than the core features, should be considered shortcuts. Using this, we present an approach to analyze the effect of shortcuts in dataset-model combination by collapsing the model into a simplistic representation for explicitly inferring using shortcuts. That is, we use the performance drop in the simplistic model, as compared to the original model, a proxy of model's reliance on the shortcuts in the dataset. Higher the drop, lesser is the reliance on shortcuts. For effective temporal understanding, the model must attend to informative tokens in both the video and text domains. Therefore, to analyze the impact of shortcuts on temporal benchmarks, we explicate the shortcuts by equally attending to all tokens. To facilitate this analysis, we introduce QUAG, a probing framework for systematically short-circuiting token-mixing operations in multi-modal self-attention blocks. 

Based on the combined model-dataset treatment of shortcuts as spurious and easy-to-learn features by \citet{murali2023shortcut}, we present an approach to analyze the effect of shortcuts by collapsing the model into a simplistic representation for explicitly inferring using shortcuts. That is, we use the performance drop in the simplistic model a proxy of model's reliance on the shortcuts. Higher the drop, lesser is the reliance on shortcuts. For effective temporal understanding, the model must attend to informative tokens in both the video and text domains. Therefore, to analyze the impact of shortcuts on temporal benchmarks, we explicate the shortcuts by equally attending to all tokens. To facilitate this analysis, we introduce QUAG, a probing framework for systematically short-circuiting token-mixing operations in multi-modal self-attention blocks. 


==> main_content/dump.tex <==
We analyze the VideoQA datasets for ambiguities and shortcuts, focusing on temporally-motivated questions. Shortcuts are spurious features in the data that are easier to learn than the \emph{core}-features necessary for generalization (\citet{geirhos2020shortcut} \citet{murali2023shortcut}). We posit that consistent shortcuts in the dataset enable the models to achieve high accuracy without even learning from the temporal video sequence. Furthermore, ambiguities in the dataset introduce noise in the core-features; inadvertently promoting the model to rely on easy-to-learn shortcuts.  

 Based on the answer-space, VideoQA datasets can be categorized as Open-ended and Multiple-choice. We choose ActivityNet-QA (\citet{yu2019activityqa}) that contains 58,000 human-annotated QA pairs on 5,800 ActivityNet videos as a representative example of open-ended VideoQA database. For multiple-choice, we select NExT-QA (\citet{xiao2021next}) that contains 47,692 5-way multiple choice questions curated from 5,440 videos.

\textbf{Open-ended Dataset}

\begin{itemize}
    \item Locality: Temporal prepositions like before and after enforce chronology. Hence, the answer of \emph{"What did the person do after <EVENT>?"} can have more than one correct answer - any action that the subject does  \emph{after} the referred instance,  but the question is annotated with a single ground truth answer. This makes learning from temporal visual features noisy and incentivize the model to rely on spurious correlations in static-visual and language domains to achieve high accuracy.   
    \item Specificity: The vocabulary of datasets can have classes at different levels of abstraction and specificity. For example, "wave", "wave hand" and "wave bye bye" are distinct answers in the answer-vocabulary of temporal questions. In other cases, like "make spaghetti" and "cook dish", both verb and nouns are abstracted. Such instances make learning and inference from core-features less reliable and unintentionally promote shortcut learning.
\end{itemize}
\textbf{Multiple-choice Dataset:}
For an 5-way multiple-choice question, the chance accuracy is ideally $ 20\% $. However, in reality, the likeliness of all the options is not the same. Since the the incorrect options are (semi) automatically curated, inadvertent shortcuts are created that discount temporal understanding:
\begin{itemize}
    \item Elimination:  it can contain out-of-context answers which are very less likely. For example, consider a question that requires temporal understanding, \emph{"What did the person do after the animal started sniffing the black item on the bed?"} with answer-options as (a) jump on it, (b) changing the diaper, (c) remove black item (d) playing with toy (e) move away. Since diaper and toy do not exist in the video, (b) and (d) can be eliminated based on the static visual information. Also, both (b) and (d) are syntactically incorrect answers and can be also eliminated by language understanding alone. Further, many action categories including jump can be inferred without temporal understanding (\citet{sevilla2021only}). Hence, based on only static and linguistic shortcuts, the probable answer pool is reduced to (c) and (e). Hence, performance on temporal questions might not be indicative of temporal understanding unless equally-likely hard-negatives are present in the answer domain.
    
\end{itemize}

While the eliminative strategy exists in open-ended VideoQA modeled as a classification task, the effect is less pronounced because of much larger answer space. 

Hence, for an ideal diagnostic dataset to confidently benchmark temporal understanding, it should have best of both -- open-ended and multiple-choice datasets. That is the answer space should be unambiguous and should contain hard-negatives that  are equally informative.





==> main_content/repro_statement.tex <==
We provide the code to implement QUAG and QUAG-attention in Appendix \ref{sec:quag_pseudo_code}. It can be easily integrated by replacing the self-attention module of the models. Also, QUAG and QUAG-attention are deterministic and non-parametric. Hence, the reproducibility of the results is ensured by reproducibility of the model codebase which we have thoroughly verified.

 We provide the scripts to curate CLAVI from Charades along with a representative subset of the dataset in the supplementary material because of licensing restrictions. We have ensured that the dataset curation code is reproducible and it will be released on GitHub under GPL3.0 license. Following the guidelines of \cite{gebru2021datasheets}, we provide a comprehensive documentation of CLAVI with the intended use in Appendix \ref{sec:datasheet}. For the finetuning experiments on CLAVI, all the experiments were repeated with three random seeds (0, 42 and 71) and the mean results reported with the standard error. We will release the finetuned checkpoints with the code on GitHub post acceptance notification. 

==> supp_material/progressive_quag.tex <==
\reba{We apply QUAG progressively to the first $n$ fusion layers of FrozenBiLM to find their relative importance in multimodality. We apply it in the step size of 4 (24 fusion blocks in total) and report the results for ActivityNet-QA (Figure \ref{fig:aqa_prog_quag}) and MSRVTT-QA (Figure \ref{fig:nqa_prog_quag}) Datasets. We consistently find that the first 8 layers are the most important in unimodal interaction and text interactions (and cross-modal interactions as well for ActivityNet-QA).}

\begin{figure}
  \centering
  \includegraphics[width=250]{images/aqa_prog_quag.png}
  \caption{Result of progressive application of QUAG on FrozenBiLM model on ActivityNet-QA dataset}
  \label{fig:aqa_prog_quag}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=250]{images/nqa_prog_quag.png}
  \caption{Result of progressive application of QUAG on FrozenBiLM model on NeXT-QA dataset}
  \label{fig:nqa_prog_quag}
\end{figure}
